Crab: A Unified Audio-Visual Scene Understanding Model with Explicit Cooperation

In recent years, numerous tasks have been proposed to encourage model to develop specified capability in understanding audio-visual scene, primarily categorized into temporal localization, spatial localization, spatio-temporal reasoning, and pixel-level understanding. Instead, human possesses a unified understanding ability for diversified tasks. Therefore, designing an audio-visual model with general capability to unify these tasks is of great value. However, simply joint training for all tasks can lead to interference due to the heterogeneity of audiovisual data and complex relationship among tasks. We argue that this problem can be solved through explicit cooperation among tasks. To achieve this goal, we propose a unified learning method which achieves explicit inter-task cooperation from both the perspectives of data and model thoroughly. Specifically, considering the labels of existing datasets are simple words, we carefully refine these datasets and construct an Audio-Visual Unified Instruction-tuning dataset with Explicit reasoning process (AV-UIE), which clarifies the cooperative relationship among tasks. Subsequently, to facilitate concrete cooperation in learning stage, an interaction-aware LoRA structure with multiple LoRA heads is designed to learn different aspects of audiovisual data interaction. By unifying the explicit cooperation across the data and model aspect, our method not only surpasses existing unified audio-visual model on multiple tasks, but also outperforms most specialized models for certain tasks. Furthermore, we also visualize the process of explicit cooperation and surprisingly find that each LoRA head has certain audio-visual understanding ability. Code and dataset: https://github.com/GeWu-Lab/Crab

==> rebuttal-exp/visual_mlm.tex <==

% \begin{table*}[htbp]
% \begin{center}

% \caption{The ablation results of explicit reasoning process (denoted as ERP) and task-aware LoRA (denoted as TA-LoRA) on MUSIC-AVQA, AVE, LLP and ARIG test set.}
% \label{tab_ablation}
% \vspace{-1em}
% \scalebox{0.8}{
% \begin{tabular}{c|cccc|c|cc|cc}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{AVQA}} & \multicolumn{1}{c|}{\textbf{AVE}} & \multicolumn{2}{c|}{\textbf{AVVP}} & \multicolumn{2}{c}{\textbf{ARIG}} \\
% & \textbf{Audio}  & \textbf{Visual} & \textbf{Audio-Visual} &\textbf{Avg} & \textbf{Acc} & \textbf{Segment-level} & \textbf{Event-level} & \textbf{cIoU} & \textbf{AUC} \\
% \hline
% \textbf{w/o. ERP}  & 75.92 & 85.63 & 71.55 & 76.05 & 78.62 & 64.89 & 62.74 & 40.92 & 0.41 \\
% \textbf{w/o. TA-LoRA} & 74.80  & 90.15  & 71.45 & 76.92 & 79.93 &  72.41 & 72.03 &  40.22 & 0.40  \\
% \textbf{Uni(Ours)} & \textbf{76.58} & \textbf{90.73} &  \textbf{74.13} & \textbf{78.94} & \textbf{81.82} & \textbf{75.25} & \textbf{75.14} & \textbf{41.78} & \textbf{0.42} \\ 

% \hline

% \end{tabular}
% }

% % \hdashline[0.5pt/3pt]
% \end{center}
% \vspace{-1.5em}
% \end{table*}


%%% 半栏
% \begin{table}[htbp]
% \belowrulesep=0pt
% \aboverulesep=0pt
% \begin{center}
% \vspace{-1em}
% \caption{Compared to visual MLMs on visual tasks.}
% \label{tab_visual_mlm}
% \vspace{-1em}
% \scalebox{0.775}{
% \begin{tabular}{c|c|c}
% % \hline
% \toprule
% \multicolumn{1}{c|}{\textbf{Method}} & \multicolumn{1}{c|}{\textbf{A-OKVQA}} & \multicolumn{1}{c}{\textbf{NExT-QA}} \\
% % &\textbf{Acc} & \textbf{Acc} \\
% \hline
% VideoLLaMA 2~\cite{cheng2024videollama} & 49.48 & 54.94 \\
% Video-ChatGPT~\cite{maaz2023video} & 54.80 & 55.92 \\
% LLaMA-VID~\cite{li2025llama} & 63.28 & 65.81 \\
% Ours(Crab) & 66.20 & 67.53 \\

% % \hline
% \bottomrule
% \end{tabular}
% }

% % \hdashline[0.5pt/3pt]
% \end{center}
% \vspace{-2em}
% \end{table}



\begin{table}[htbp]
\belowrulesep=0pt
\aboverulesep=0pt
\begin{center}
\vspace{-1.2em}
\caption{Compared to visual MLMs on visual tasks.}
\label{tab_visual_mlm}
\vspace{-1em}
\scalebox{0.6}{
\begin{tabular}{c|c|c|c|c}
% \hline
\toprule
\multicolumn{1}{c|}{\textbf{Method}} & \multicolumn{1}{c|}{VideoLLaMA 2} & \multicolumn{1}{c|}{Video-ChatGPT} & \multicolumn{1}{c|}{LLaMA-VID} & \multicolumn{1}{c}{\textbf{Ours(Crab)}} \\
% &\textbf{Acc} & \textbf{Acc} \\
\hline
A-OKVQA & 49.48 & 54.80 & 63.28 & \textbf{66.20} \\
NExT-QA & 54.94 & 55.92 & 65.81 & \textbf{67.53} \\

% \hline
\bottomrule
\end{tabular}
}

% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-2.5em}
\end{table}



==> sec/tables/hyper_parameters.tex <==
\begin{table}[h]
\begin{center}
\caption{hyper parameters}
\label{tab_hyper_para}
\scalebox{0.8}{
\begin{tabular}{c|c}
\hline
\textbf{parameter} & \textbf{value} \\
\hline
% \textbf{AVEL}～\cite{tian2018audio} & 72.70 \\
% \textbf{DAM}~\cite{wu2019dual} & 74.50 \\ 
\textbf{AVIN}~\cite{lin2019dual} & 75.20 \\
\textbf{AVT}~\cite{lin2020audiovisual} & 75.80 \\
\textbf{CMRAN}~\cite{xu2020cross} & 77.40 \\
\textbf{MPN}~\cite{yu2021mpn} & 77.60 \\
\textbf{PSP}~\cite{zhou2021positive} & \underline{77.80} \\
\textbf{MM-Pyramid}~\cite{yu2022mm} & \underline{77.80} \\ 
\hline
\textbf{AV-Unified(Ours)} & \textbf{81.82} \\ 
\hline
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\end{table}



==> sec/tables/table_ablation_arig.tex <==
\begin{table}[h]
\begin{center}
\caption{The ablation results on our spatial localization test set.}
\label{tab_ablation_arig}
\vspace{-1em}
\scalebox{0.8}{
\begin{tabular}{c|cc}
\hline
\textbf{Method} & \textbf{cIoU} & \textbf{AUC} \\
\hline
% \textbf{FNAC}~\cite{sun2023learning} & 27.15 & 0.31 \\
% \hline
\textbf{w/o. reasoning process} & 40.92 & 0.41 \\
\textbf{w/o. task-aware LoRA} & 40.22 & 0.40 \\
\hline
\textbf{AV-Unified(Ours)} & \textbf{41.78} & \textbf{0.42} \\ 

\hline

\end{tabular}
}

% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-2em}
\end{table}




==> sec/tables/table_ablation_ave.tex <==
\begin{table}[h]
\begin{center}

\caption{The ablation results on AVE fully supervised dataset.}
\label{tab_ablation_ave}

\scalebox{0.8}{
\begin{tabular}{c|c}
\hline
\textbf{Method} & \textbf{Acc} \\
\hline
% \textbf{MM-Pyramid}~\cite{yu2022mm} & \underline{77.80} \\ 
% \hline
\textbf{w/o. reasoning process} & 78.62 \\
\textbf{w/o. task-aware LoRA} & 79.93 \\ 
\hline
\textbf{AV-Unified(Ours)} & 81.82 \\ 

\hline

\end{tabular}
}


% \hdashline[0.5pt/3pt]
\end{center}
\end{table}



==> sec/tables/table_ablation_ave_avvp.tex <==

\begin{table}[ht]
\centering
\caption{The experiment results on AVE fully supervised dataset and LLP dataset.}
\label{tab_ablation_ave_avvp}
\vspace{-1em}
\scalebox{0.8}{
\begin{tabular}{c|c|cc}
\hline
\multirow{2}{*}{\textbf{Method}} & \textbf{AVE task} & \multicolumn{2}{c}{\textbf{AVVP task}} \\
& \textbf{Acc} & \textbf{Segment-level} & \textbf{Event-level} \\
\hline
\textbf{w/o. reasoning process} & 78.62 & 64.89 & 62.74 \\
\textbf{w/o. task-aware LoRA} & 79.93 &  72.41 & 72.03 \\ 
\hline
\textbf{AV-Unified(Ours)} & \textbf{81.82} & \textbf{75.25} & \textbf{75.14} \\
\hline
\end{tabular}
}
\vspace{-1.5em}
\end{table}



==> sec/tables/table_ablation_avqa.tex <==
\begin{table}[htbp]
\begin{center}

\caption{The ablation results on MUSIC-AVQA dataset.}
\label{tab_ablation_avqa}
\vspace{-1em}
\scalebox{0.925}{
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Method} & \textbf{A}  & \textbf{V} & \textbf{A-V} &\textbf{Avg}  \\
\hline
% \textbf{TSPM}~\cite{li2024boosting} & \underline{84.07} & 64.65 & \textbf{76.91} & \underline{82.29} & \underline{84.90} & \underline{83.61} & 82.19 & \underline{76.21} & \underline{71.85} & \textbf{65.76} & \textbf{71.17} & \underline{73.51} & \underline{76.79} \\
% \hline
\textbf{w/o. reasoning process}  & 75.92 & 85.63 & 71.55 & 76.05 \\
\textbf{w/o. task-aware LoRA} & 74.80  & 90.15  & 71.45 & 76.92 \\
\textbf{AV-Unified(Ours)} & \textbf{76.58} & \textbf{90.73} &  \textbf{74.13} & \textbf{78.94} \\ 

\hline

\end{tabular}
}

% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-2em}
\end{table}



==> sec/tables/table_ablation_avs.tex <==
\begin{table}[htbp]
\begin{center}

\caption{The ablation results on AVS-Bench dataset.}
\label{tab_ablation_avs}

\scalebox{0.6}{
\begin{tabular}{c|c|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{Visual Backbone}} &    
\multicolumn{2}{c|}{\textbf{S4}} &         
\multicolumn{2}{c|}{\textbf{MS3}} &         
\multicolumn{2}{c}{\textbf{AVSS}}  
\\
& & \textbf{miou} & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{miou} & \textbf{F-score}   \\
\hline
% \textbf{AVSegFormer}~\cite{gao2024avsegformer} & \textbf{PVT-v2} & \textbf{82.10} & \textbf{89.90} & 58.40 & \textbf{69.30} & \textbf{36.70} & \textbf{42.00} \\
% \hline
\textbf{w/o. reasoning process} & ViT/L-14 & 70.83  & 82.01 & 56.43 & 65.91 & 25.35 & 37.01 \\
\textbf{w/o. task-aware LoRA} & ViT/L-14 & 69.72 & 76.31 & 53.92 & 60.31 &  23.61 & 31.87 \\
\hline
\textbf{AV-Unified(Ours)} & ViT/L-14 & 71.00 & 82.30 & 56.30 & 65.87 & 26.00 & 36.30  \\ 

\hline

\end{tabular}
}


% \hdashline[0.5pt/3pt]
\end{center}
\end{table}



==> sec/tables/table_ablation_avs_ref_avs.tex <==
% \begin{table*}[htbp]
% \begin{center}
% \caption{The ablation results of explicit reasoning process (denoted as ERP) and task-aware LoRA (denoted as TA-LoRA) on AVS-Bench and Ref-AVS test set.}
% \label{tab_ablation_avs_ref_avs}
% \vspace{-1.0em}
% \scalebox{0.8}{
% \begin{tabular}{c|cc|cc|cc|cc|cc|c}
% \hline
% \multirow{2}{*}{\textbf{Method}} & 
% % \multirow{2}{*}{\textbf{Visual Backbone}} &    
% \multicolumn{2}{c|}{\textbf{S4}} &         
% \multicolumn{2}{c|}{\textbf{MS3}} &         
% \multicolumn{2}{c|}{\textbf{AVSS}} &
% \multicolumn{2}{c|}{\textbf{Seen}} &
% \multicolumn{2}{c|}{\textbf{Unseen}} & 
% \textbf{Null}
% \\
% & \textbf{miou} & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{miou} & \textbf{F-score} & \textbf{miou} & \textbf{F-score} & \textbf{S($\downarrow$)} \\
% \hline
% \textbf{w/o. ERP} & 73.13  & 86.51 & \textbf{58.43} & \textbf{66.91} & 25.43 & 31.93 & 40.34 & \textbf{0.58} & 45.12 & 0.54 & 0.02 \\
% \textbf{w/o. TA-LoRA} & 72.72 & 86.03 & 56.92 & 64.31 & 24.57 & 31.28 & 39.22 & 0.56 & 45.01 & 0.60 & 0.08 \\
% \hline
% \textbf{Uni(Ours)}& \textbf{73.25} & \textbf{86.81} & 58.21 & 66.24 & \textbf{26.52} & \textbf{32.10} & \textbf{40.54} & \textbf{0.58} & \textbf{45.55} & \textbf{0.63} & \textbf{0.01} \\ 
% \hline
% \end{tabular}
% }
% % \hdashline[0.5pt/3pt]
% \end{center}
% \vspace{-1.25em}
% \end{table*}



\begin{table}[htbp]
\begin{center}
\caption{The ablation results of explicit reasoning process (denoted as ERP) and task-aware LoRA (denoted as TA-LoRA) on AVS-Bench and Ref-AVS test set.}
\label{tab_ablation_avs_ref_avs}
\vspace{-1.0em}
\scalebox{0.8}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Method}} & 
% \multirow{2}{*}{\textbf{Visual Backbone}} &    
\multicolumn{1}{c|}{\textbf{S4}} &         
\multicolumn{1}{c|}{\textbf{MS3}} &         
\multicolumn{1}{c|}{\textbf{AVSS}} &
\multicolumn{1}{c|}{\textbf{Seen}} &
\multicolumn{1}{c|}{\textbf{Unseen}} & 
\textbf{Null}
\\
& \textbf{miou} & \textbf{miou} & \textbf{miou} & \textbf{miou} & \textbf{miou} & \textbf{S($\downarrow$)} \\
\hline
w/o. ERP & 73.13  & \textbf{58.43} & 25.43 & 40.34 & 45.12 & 0.02 \\
w/o. TA-LoRA & 72.72 & 56.92 & 24.57 & 39.22 & 45.01 & 0.08 \\
\hline
\textbf{Crab(Ours)}& \textbf{73.25} & 58.21 & \textbf{26.52} & \textbf{40.54} & \textbf{45.55} & \textbf{0.01} \\ 
\hline
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-1.25em}
\end{table}








==> sec/tables/table_ablation_avvp.tex <==
\begin{table}[h]
\begin{center}

\caption{AVVP ablation results}
\label{tab_ablation_avvp}

\scalebox{0.8}{
\begin{tabular}{c|c|c}
\hline
\textbf{Method} & \textbf{Segment-level} & \textbf{Event-level} \\
\hline
% \textbf{CMPAE}~\cite{gao2023collecting} & \underline{59.20} & \underline{51.80} \\
% \hline
\textbf{w/o. reasoning process} & 64.89 & 62.74 \\
\textbf{w/o. task-aware LoRA} &  72.41 & 72.03  \\ 
\hline
\textbf{AV-Unified(Ours)} & 74.70 & 74.60 \\ 

\hline

\end{tabular}
}


% \hdashline[0.5pt/3pt]
\end{center}
\end{table}



==> sec/tables/table_ablation_ref_avs.tex <==
\begin{table}[htbp]
\begin{center}

\caption{The ablation results of explicit reasoning process (denoted as ERP) and task-aware LoRA (denoted as TA-LoRA) on AVS-Bench and Ref-AVS test set.}
\label{tab_ablation_ref_avs}

\scalebox{0.75}{
\begin{tabular}{c|cc|cc|cc|c}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Seen}} &
\multicolumn{2}{c|}{\textbf{Unseen}} & \multicolumn{2}{c|}{\textbf{Mix(S+U)}} & \textbf{Null}
\\
& \textbf{miou} & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{miou} & \textbf{F-score} & \textbf{S($\downarrow$)}  \\
\hline
% \textbf{EEMC}~\cite{wang2024ref} & 34.20 & 0.51 & \textbf{49.54} & \textbf{0.65} & \underline{41.87} & \underline{0.58} & 0.01 \\ 
% \hline
\textbf{w/o. ERP} & 40.34 & 0.58 & 45.12 & 0.54 & 43.10 & 0.63 & 0.26 \\
\textbf{w/o. T-A LoRA} & 39.22 & 0.56 & 45.01 & 0.60 & 42.43 & 0.54 & 0.25 \\
\hline
\textbf{AV-Unified(Ours)} & 40.54 & 0.58 & 45.55 & 0.63 & 43.05 & 0.61 & 0.27 
\\
\hline

\end{tabular}
}


% \hdashline[0.5pt/3pt]
\end{center}
\end{table}



==> sec/tables/table_ave.tex <==
\begin{table}[h]
\begin{center}
\caption{The experiment results on AVE fully supervised dataset.}
\label{tab_ave}
\scalebox{0.8}{
\begin{tabular}{c|c}
\hline
\textbf{Method} & \textbf{Acc} \\
\hline
% \textbf{AVEL}～\cite{tian2018audio} & 72.70 \\
% \textbf{DAM}~\cite{wu2019dual} & 74.50 \\ 
\textbf{AVIN}~\cite{lin2019dual} & 75.20 \\
\textbf{AVT}~\cite{lin2020audiovisual} & 75.80 \\
\textbf{CMRAN}~\cite{xu2020cross} & 77.40 \\
\textbf{MPN}~\cite{yu2021mpn} & 77.60 \\
\textbf{PSP}~\cite{zhou2021positive} & \underline{77.80} \\
\textbf{MM-Pyramid}~\cite{yu2022mm} & \underline{77.80} \\ 
\hline
\textbf{AV-Unified(Ours)} & \textbf{81.82} \\ 
\hline
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\end{table}

==> sec/tables/table_avs.tex <==
% \begin{table}[htbp]
% \begin{center}
% \caption{The experiment results on AVS-Bench dataset.}
% \label{tab_avs}
% \scalebox{0.6}{
% \begin{tabular}{c|c|cc|cc|cc}
% \hline
% \multirow{2}{*}{\textbf{Method}} & 
% \multirow{2}{*}{\textbf{Visual Backbone}} &    
% \multicolumn{2}{c|}{\textbf{S4}} &         
% \multicolumn{2}{c|}{\textbf{MS3}} &         
% \multicolumn{2}{c}{\textbf{AVSS}}  
% \\
% & & \textbf{miou} & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{miou} & \textbf{F-score}   \\
% \hline
% \textbf{LVS} & \textbf{ResNet-50} & 37.90 & 51.00 & 29.50 & 33.00 & —— & —— \\
% \textbf{MSSL}~\cite{qian2020multiple} & \textbf{ResNet-18} & 44.90 & 66.30 & 26.10 & 36.30 & —— & —— \\
% \textbf{3DC} & \textbf{ResNet-34} & 57.10 & 75.90 & 36.90 & 50.30 & 17.30 & 21.60 \\
% \textbf{SST}~\cite{duke2021sstvos} & \textbf{ResNet-101} & 66.30 & 80.10 & 42.60 & 57.20 & —— & —— \\
% \textbf{iGAN}~\cite{mao2021transformer} & \textbf{Swin-T} & 61.60 & 77.80 & 42.90 & 54.40 & —— & —— \\
% \textbf{LGVT}~\cite{zhang2021learning} & \textbf{Swin-T} & 74.90 & 87.30 & 40.70 & 59.30 & —— & —— \\
% \textbf{TPAVI}~\cite{zhou2022audio} & \textbf{ResNet-50} & 72.80 & 84.80 & 47.90 & 57.80 & 20.20 & 25.20 \\
% % \textbf{CATR}~\cite{li2023catr} & \textbf{ResNet-50} & 74.80 & 86.60 & 52.80 & 65.30 & —— & —— \\
% % \textbf{BAVS}~\cite{liu2024bavs} & \textbf{ResNet-50} & 78.00 & 85.30 & 50.20 & 62.40 & 24.70 & 29.60 \\
% % \textbf{AVSegFormer}~\cite{gao2024avsegformer} & \textbf{ResNet-50} & 76.50 & 85.90 & 49.50 & 62.80 & 24.90 & 29.30 \\
% \textbf{TPAVI}~\cite{zhou2022audio} & \textbf{PVT-v2} & 78.70 & 87.90 & 54.00 & 64.50 & 29.80 & 35.20 \\
% % \textbf{CATR}~\cite{li2023catr} & \textbf{PVT-v2} & 81.40 & \underline{89.60} & \textbf{59.00} & \underline{67.00} & —— & —— \\
% % \textbf{BAVS}~\cite{liu2024bavs} & \textbf{PVT-v2} & \underline{82.00} & 88.60 & \underline{58.60} & 65.50 & \underline{32.60} & \underline{36.40} \\
% % \textbf{AVSegFormer}~\cite{gao2024avsegformer} & \textbf{PVT-v2} & \textbf{82.10} & \textbf{89.90} & 58.40 & \textbf{69.30} & \textbf{36.70} & \textbf{42.00} \\
% \hline
% \textbf{AV-Unified(Ours)} & \textbf{ViT/L-14} & 71.00 & 82.30 & 56.30 & 65.87 & 26.00 & 36.30  \\ 
% \hline
% \end{tabular}
% }
% % \hdashline[0.5pt/3pt]
% \end{center}
% \end{table}




\begin{table}[htbp]
\begin{center}
\caption{The experiment results on AVS-Bench dataset.}
\label{tab_avs}
\scalebox{0.8}{
\begin{tabular}{c|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} &     
\multicolumn{2}{c|}{\textbf{S4}} &         
\multicolumn{2}{c|}{\textbf{MS3}} &         
\multicolumn{2}{c}{\textbf{AVSS}}  
\\
& \textbf{miou} & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{miou} & \textbf{F-score}   \\
\hline
\textbf{LVS}  & 37.90 & 51.00 & 29.50 & 33.00 & —— & —— \\
\textbf{MSSL}~\cite{qian2020multiple} & 44.90 & 66.30 & 26.10 & 36.30 & —— & —— \\
\textbf{3DC} & 57.10 & 75.90 & 36.90 & 50.30 & 17.30 & 21.60 \\
\textbf{SST}~\cite{duke2021sstvos} & 66.30 & 80.10 & 42.60 & 57.20 & —— & —— \\
\textbf{iGAN}~\cite{mao2021transformer} & 61.60 & 77.80 & 42.90 & 54.40 & —— & —— \\
\textbf{LGVT}~\cite{zhang2021learning} & 74.90 & 87.30 & 40.70 & 59.30 & —— & —— \\
\textbf{TPAVI}~\cite{zhou2022audio} & 72.80 & 84.80 & 47.90 & 57.80 & 20.20 & 25.20 \\
% \textbf{CATR}~\cite{li2023catr} & \textbf{ResNet-50} & 74.80 & 86.60 & 52.80 & 65.30 & —— & —— \\
% \textbf{BAVS}~\cite{liu2024bavs} & \textbf{ResNet-50} & 78.00 & 85.30 & 50.20 & 62.40 & 24.70 & 29.60 \\
% \textbf{AVSegFormer}~\cite{gao2024avsegformer} & \textbf{ResNet-50} & 76.50 & 85.90 & 49.50 & 62.80 & 24.90 & 29.30 \\
\textbf{TPAVI}~\cite{zhou2022audio} & 78.70 & 87.90 & 54.00 & 64.50 & 29.80 & 35.20 \\
% \textbf{CATR}~\cite{li2023catr} & \textbf{PVT-v2} & 81.40 & \underline{89.60} & \textbf{59.00} & \underline{67.00} & —— & —— \\
% \textbf{BAVS}~\cite{liu2024bavs} & \textbf{PVT-v2} & \underline{82.00} & 88.60 & \underline{58.60} & 65.50 & \underline{32.60} & \underline{36.40} \\
% \textbf{AVSegFormer}~\cite{gao2024avsegformer} & \textbf{PVT-v2} & \textbf{82.10} & \textbf{89.90} & 58.40 & \textbf{69.30} & \textbf{36.70} & \textbf{42.00} \\
\hline
\textbf{AV-Unified(Ours)} & 71.00 & 82.30 & 56.30 & 65.87 & 26.00 & 36.30  \\ 
\hline
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\end{table}

==> sec/tables/table_avvp.tex <==
\begin{table}[h]
\begin{center}
\caption{The experiment results on LLP dataset.}
\label{tab_avvp}
\scalebox{0.8}{
\begin{tabular}{c|c|c}
\hline
\textbf{Method} & \textbf{Segment-level} & \textbf{Event-level} \\
\hline
% \textbf{AVEL}~\cite{tian2018audio} & 35.40 & 31.60 \\
% \textbf{AVSDN}~\cite{lin2019dual} & 37.10 & 26.50 \\ 
% \textbf{HAN}~\cite{tian2020unified} & 48.90 & 43.00 \\
\textbf{MA}~\cite{wu2021exploring} & 55.10 & 49.00 \\
\textbf{CVCMS}~\cite{lin2021exploring} & 57.00 & 49.50 \\
\textbf{DHHN}~\cite{jiang2022dhhn} & 56.80 & 49.40 \\
\textbf{MM-Pyramid}~\cite{yu2022mm} & 55.80 & 49.40 \\
\textbf{CMPAE}~\cite{gao2023collecting} & \underline{59.20} & \underline{51.80} \\
\textbf{Meerkat}~\cite{chowdhury2024meerkat} & 54.96 & —— \\
\hline
\textbf{AV-Unified(Ours)} & \textbf{59.00} & \textbf{54.44} \\ 
\hline
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\end{table}

==> sec/tables/table_ref_avs.tex <==
% \begin{table}[htbp]
% \begin{center}
% \caption{The experiemnt results on Ref-AVS dataset.}
% \label{tab_ref_avs}
% \scalebox{0.8}{
% \begin{tabular}{c|cc|cc|cc|c}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Seen}} &
% \multicolumn{2}{c|}{\textbf{Unseen}} & \multicolumn{2}{c|}{\textbf{Mix(S+U)}} & \textbf{Null}
% \\
%  & \textbf{miou} & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{miou} & \textbf{F-score} & \textbf{S}  \\
% \hline
% % \textbf{AVSBench}~\cite{zhou2022audio} & 21.22 & 0.46 & 27.67 & 0.51 & 24.45 & 0.48 & —— \\
% % \textbf{AVSBench+text}~\cite{zhou2022audio} & 23.20 & 0.51 & 32.36 & 0.55 & 27.78 & 0.53 & 0.21 \\
% % \textbf{AVSegFormer}~\cite{gao2024avsegformer} & 29.16 & 0.42 & 32.71 & 0.45 & 30.94 & 0.44 & —— \\
% % \textbf{AVSegFormer+text}~\cite{gao2024avsegformer} & 33.47 & 0.47 & 36.05 & 0.50 & 34.76 & 0.49 & 0.17 \\
% \textbf{GAVS}~\cite{wang2024prompting} & 24.85 & 0.46 & 27.86 & 0.46 & 26.36 & 0.46 & —— \\
% \textbf{GAVS+text}~\cite{wang2024prompting} & 28.93 & 0.50 & 29.82 & 0.50 & 29.38 & 0.50 & 0.19 \\
% \textbf{ReferFormer}~\cite{wu2022language} & 27.46 & 0.48 & 24.94 & 0.50 & 26.20 & 0.49 & —— \\
% \textbf{ReferFormer+audio}~\cite{wu2022language} & 31.31 & 0.50 & 30.40 & 0.49 & 30.86 & 0.50 & 0.18 \\
% \textbf{R2VOS}~\cite{li2023robust} & 21.34 & 0.31 & 23.91 & 0.43 & 22.63 & 0.37 & —— \\
% \textbf{R2VOS+audio}~\cite{li2023robust} & 25.01 & 0.41 & 27.93 & 0.50 & 26.47 & 0.45 & 0.18 \\
% \textbf{EEMC}~\cite{wang2024ref} & 34.20 & 0.51 & \textbf{49.54} & \textbf{0.65} & \underline{41.87} & \underline{0.58} & 0.01 \\ 
% \hline
% \textbf{AV-Unified(Ours)} & \textbf{40.54} & \textbf{0.58} & \underline{45.55} & \underline{0.63} & \textbf{43.05} & \textbf{0.61} & 0.27 
% \\
% \hline
% \end{tabular}
% }
% % \hdashline[0.5pt/3pt]
% \end{center}
% \end{table}

\begin{table}[htbp]
\begin{center}
\caption{The experiemnt results on Ref-AVS dataset.}
\label{tab_ref_avs}
\scalebox{0.8}{
\begin{tabular}{c|cc|cc|c}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Seen}} &
\multicolumn{2}{c|}{\textbf{Unseen}} & \textbf{Null}
\\
& \textbf{miou} & \textbf{F-score} & \textbf{miou}  & \textbf{F-score} & \textbf{S}  \\
\hline
\textbf{AVSBench}~\cite{zhou2022audio} & 21.22 & 0.46 & 27.67 & 0.51 & 24.45 & 0.48 & —— \\
\textbf{AVSBench+text}~\cite{zhou2022audio} & 23.20 & 0.51 & 32.36 & 0.55 & 27.78 & 0.53 & 0.21 \\
\textbf{AVSegFormer}~\cite{gao2024avsegformer} & 29.16 & 0.42 & 32.71 & 0.45 & 30.94 & 0.44 & —— \\
\textbf{AVSegFormer+text}~\cite{gao2024avsegformer} & 33.47 & 0.47 & 36.05 & 0.50 & 34.76 & 0.49 & 0.17 \\
\textbf{GAVS}~\cite{wang2024prompting} & 24.85 & 0.46 & 27.86 & 0.46 & —— \\
\textbf{GAVS+text}~\cite{wang2024prompting} & 28.93 & 0.50 & 29.82 & 0.50 & 0.19 \\
\textbf{ReferFormer}~\cite{wu2022language} & 27.46 & 0.48 & 24.94 & 0.50 & —— \\
\textbf{ReferFormer+audio}~\cite{wu2022language} & 31.31 & 0.50 & 30.40 & 0.49 & 0.18 \\
\textbf{R2VOS}~\cite{li2023robust} & 21.34 & 0.31 & 23.91 & 0.43 & —— \\
\textbf{R2VOS+audio}~\cite{li2023robust} & 25.01 & 0.41 & 27.93 & 0.50 & 0.18 \\
\textbf{EEMC}~\cite{wang2024ref} & 34.20 & 0.51 & \textbf{49.54} & \textbf{0.65} & 0.01 \\ 
\hline
\textbf{Uni} & \textbf{40.54} & \textbf{0.58} & \underline{45.55} & \underline{0.63} & 0.27 
\\
\hline
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\end{table}

==> sec/tables/test.tex <==
\begin{tabular}{c|ccc|ccc}
\bottomrule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{CREMA-D}}  & \multicolumn{3}{c}{MMPareto}  \\ 
& \textbf{75.13}    & \textbf{65.46}   & 55.24   & \textbf{70.13}        & \textbf{56.40}   & \textbf{53.05} \\ 
\toprule
\end{tabular}

